A spectral element solution of the 2D linearized potential flow radiation problem

We present a scalable 2D Galerkin spectral element method solution to the linearized potential flow radiation problem for wave induced forcing of a floating offshore structure. The pseudo-impulsive formulation of the problem is solved in the time-domain using a Gaussian displacement signal tailored to the discrete resolution. The added mass and damping coefficients are then obtained via Fourier transformation. The spectral element method is used to discretize the spatial fluid domain, whereas the classical explicit 4-stage 4th order Runge-Kutta scheme is employed for the temporal integration. Spectral convergence of the proposed model is established for both affine and curvilinear elements, and the computational effort is shown to scale with $\mathcal{O}(N^p)$, with $N$ begin the total number of grid points and $p \approx 1$. Temporal stability properties, caused by the spatial resolution, are considered to ensure a stable model. The solver is used to compute the hydrodynamic coefficients for several floating bodies and compare against known public benchmark results. The results are showing excellent agreement, ultimately validating the solver and emphasizing the geometrical flexibility and high accuracy and efficiency of the proposed solver strategy. Lastly, an extensive investigation of non-resolved energy from the pseudo-impulse is carried out to characterise the induced spurious oscillations of the free surface quantities leading to a verification of a proposal on how to efficiently and accurately calculate added mass and damping coefficients in pseudo-impulsive solvers.

==> references.tex <==
\bibitem{bingham2017supplemental}Bingham, H. Supplemental Lecture Note for: Wave Loads on Ships and Offshore Structures. {\em Lecture Note For 41222}. (2017)
\bibitem{bingham2018wavegeneration}Bingham, H. A note on wave generation and absorption in numerical wave tanks. (Technical University of Denmark, Section of Coastal, Structural,2018)
\bibitem{christensen2012differentialligninger}Christensen, O. Differentialligninger og uendelige rækker. (Technical University of Denmark,2012)
\bibitem{cheney2012numerical}Cheney, E. \& Kincaid, D. Numerical mathematics and computing. (Cengage Learning,2012)
\bibitem{canuto2007spectral}Canuto, C., Hussaini, M., Quarteroni, A. \& Zang, T. Spectral methods: fundamentals in single domains. (Springer Science & Business Media,2007)
\bibitem{canuto2007spectral_evolution}Canuto, C., Hussaini, M., Quarteroni, A. \& Zang, T. Spectral methods: evolution to complex geometries and applications to fluid dynamics. (Springer Science & Business Media,2007)
\bibitem{engsig2013fast}Engsig-Karup, A., Glimberg, S., Nielsen, A. \& Lindberg, O. Fast hydrodynamics on heterogenous many-core hardware. {\em Designing Scientific Applications On GPUs}. pp. 251-294 (2013)
\bibitem{engsig2009spectral}Engsig-Karup, A. The Spectral/hp-Finite Element Method for Partial Differential Equations. {\em Lecture Note For 02623}. (2009)
\bibitem{hesthaven2007nodal}Hesthaven, J. \& Warburton, T. Nodal discontinuous Galerkin methods: algorithms, analysis, and applications. (Springer Science & Business Media,2007)
\bibitem{hesthaven2007spectral}Hesthaven, J., Gottlieb, S. \& Gottlieb, D. Spectral methods for time-dependent problems. (Cambridge University Press,2007)
\bibitem{karniadakis2005spectral}Karniadakis, G. \& Sherwin, S. Spectral/hp element methods for computational fluid dynamics. (OUP Oxford,2005)
\bibitem{kopriva2009implementing}Kopriva, D. Implementing spectral methods for partial differential equations: Algorithms for scientists and engineers. (Springer Science & Business Media,2009)
\bibitem{leveque2007finite}LeVeque, R. Finite difference methods for ordinary and partial differential equations: steady-state and time-dependent problems. (SIAM,2007)
\bibitem{madsen2016firstorder}Madsen, P. A note on stokes first order theory. {\em Lecture Note For 41224}. (2016)
\bibitem{madsen2007time}Madsen, H. Time series analysis. (Chapman,2007)
\bibitem{svendsen1976hydrodynamics}Svendsen, I. \& Jonsson, I. Hydrodynamics of coastal regions. (Den Private ingeniørfond, Technical University of Denmark,1976)
\bibitem{sommerfeld1949partial}Sommerfeld, A. Partial differential equations in physics. (Academic press,1949)
\bibitem{amini2017solving}Amini-Afshar, M. \& Bingham, H. Solving the linearized forward-speed radiation problem using a high-order finite difference method on overlapping grids. {\em Applied Ocean Research}. \textbf{69} pp. 220-244 (2017,12)
\bibitem{amini2018pseudo}Amini-Afshar, M. \& Bingham, H. Pseudo-impulsive solutions of the forward-speed diffraction problem using a high-order finite-difference method. {\em Applied Ocean Research}. \textbf{80} pp. 197-219 (2018,11)
\bibitem{babarit2015theoretical}Babarit, A. \& Delhommeau, G. Theoretical and numerical aspects of the open source BEM solver NEMOH. {\em 11th European Wave And Tidal Energy Conference (EWTEC2015)}. (2015,9), https://hal.archives-ouvertes.fr/hal-01198800
\bibitem{bingham2007accuracy}Bingham, H. \& Zhang, H. On the accuracy of finite-difference solutions for nonlinear water waves. {\em Journal Of Engineering Mathematics}. \textbf{58} pp. 211-228 (2007,8)
\bibitem{bingham2008efficient}Bingham, H. \& Engsig-Karup, A. Efficient Solution of the 3D Laplace Problem for Nonlinear Wave-Structure Interaction. {\em Proceedings Of The International Conference On Offshore Mechanics And Arctic Engineering - OMAE}. \textbf{6} (2008,1)
\bibitem{butcher1996history}Butcher, J. A history of Runge-Kutta methods. {\em Applied Numerical Mathematics}. \textbf{20}, 247-260 (1996), https://www.sciencedirect.com/science/article/pii/0168927495001085
\bibitem{borsboom2021generating}Borsboom, M. \& Jacobsen, N. A generating-absorbing boundary condition for dispersive waves. {\em International Journal For Numerical Methods In Fluids}. \textbf{93}, 2443-2467 (2021), https://onlinelibrary.wiley.com/doi/abs/10.1002/fld.4982
\bibitem{CuthillMckee}Cuthill, E. \& McKee, J. Reducing the Bandwidth of Sparse Symmetric Matrices. {\em Proceedings Of The 1969 24th National Conference}. pp. 157-172 (1969), https://doi.org/10.1145/800195.805928
\bibitem{cooley1965algorithm}Cooley, J. \& Tukey, J. An algorithm for the machine calculation of complex Fourier series. {\em Mathematics Of Computation}. \textbf{19}, 297-301 (1965)
\bibitem{davidson2020efficient}Davidson, J. \& Costello, R. Efficient Nonlinear Hydrodynamic Models for Wave Energy Converter Design—A Scoping Study. {\em Journal Of Marine Science And Engineering}. \textbf{8} (2020), https://www.mdpi.com/2077-1312/8/1/35
\bibitem{ducrozet2010high}Ducrozet, G., Bingham, H., Engsig-Karup, A. \& Ferrant, P. High-Order Finite Difference Solution for 3D Nonlinear Wave-Structure Interaction. {\em Journal Of Hydrodynamics}. \textbf{22} pp. 225-230 (2010,10)
\bibitem{engsig2019mixed}Engsig-Karup, A., Monteserin, C. \& Eskilsson, C. A Stabilised Mixed Eulerian Lagrangian Spectral Element Method for Nonlinear Wave Interaction with Fixed Structures. {\em Water Waves}. \textbf{1} pp. 315-342 (2019,11)
\bibitem{engsig2016stabilised}Engsig-Karup, A., Eskilsson, C. \& Bigoni, D. A stabilised nodal spectral element method for fully nonlinear water waves. {\em Journal Of Computational Physics}. \textbf{318} pp. 1-21 (2016), https://www.sciencedirect.com/science/article/pii/S0021999116301255
\bibitem{engsig2018spectral}Engsig-Karup, A. \& Eskilsson, C. Spectral Element FNPF Simulation of Focused Wave Groups Impacting a Fixed FPSO-type Body. {\em International Journal Of Offshore And Polar Engineering}. \textbf{29} pp. 141-148 (2019,6)
\bibitem{engsig2009efficient}Engsig-Karup, A., Bingham, H. \& Lindberg, O. An efficient flexible-order model for 3D nonlinear water waves. {\em Journal Of Computational Physics}. \textbf{228}, 2100-2118 (2009), https://www.sciencedirect.com/science/article/pii/S0021999108006190
\bibitem{engsig2021efficient}Engsig-Karup, A. \& Laskowski, W. An efficient p-multigrid spectral element model for fully nonlinear water waves and fixed bodies. {\em International Journal For Numerical Methods In Fluids}. \textbf{93}, 2823-2841 (2021), https://onlinelibrary.wiley.com/doi/abs/10.1002/fld.5011
\bibitem{esmaeilzadeh2019shape}Esmaeilzadeh, S. \& Alam, M. Shape optimization of wave energy converters for broadband directional incident waves. {\em Ocean Engineering}. \textbf{174} pp. 186-200 (2019), https://www.sciencedirect.com/science/article/pii/S0029801818308564
\bibitem{guler2022reduced}Güler Eroğlu, F., Mücke, N. \& Engsig-Karup, A. Reduced Order Modelling for Dispersive and Nonlinear Water Wave Modelling. {\em 37<sup>th</sup> International Workshop On Water Waves And Floating Bodies}. (2022)
\bibitem{gordon1973transfinite}Gordon, W. \& Hall, C. Transfinite element methods: blending-function interpolation over arbitrary curved element domains. {\em Numerische Mathematik}. \textbf{21}, 109-129 (1973)
\bibitem{gordon1973construction}Gordon, W. \& Hall, C. Construction of curvilinear co-ordinate systems and applications to mesh generation. {\em International Journal For Numerical Methods In Engineering}. \textbf{7}, 461-477 (1973), https://onlinelibrary.wiley.com/doi/abs/10.1002/nme.1620070405
\bibitem{hulme1982wave}Hulme, A. The wave forces acting on a floating hemisphere undergoing forced periodic oscillations. {\em Journal Of Fluid Mechanics}. \textbf{121} pp. 443-463 (1982)
\bibitem{haskind1946hydrodynamic}Haskind, M. The hydrodynamic theory of ship oscillations in rolling and pitching. {\em Prikl. Mat. Mekh}. \textbf{10} pp. 33-66 (1946)
\bibitem{jiang2012precorrected}Jiang, S., Teng, B., Gou, Y. \& Ning, D. A precorrected-FFT higher-order boundary element method for wave–body problems. {\em Engineering Analysis With Boundary Elements}. \textbf{36}, 404-415 (2012)
\bibitem{kara2011prediction}Kara, F. Time domain prediction of added resistance of ships. {\em Journal Of Ship Research}. \textbf{55}, 163-184 (2011)
\bibitem{kontos2016nonlinear}Kontos, S., Bingham, H., Lindberg, O. \& Engsig-Karup, A. On nonlinear wave-structure interaction using an immersed boundary method in 2D.. {\em 31<sup>th</sup> International Workshop On Water Waves And Floating Bodies}. (2016)
\bibitem{korsmeyer1998forward}Korsmeyer, F. \& Bingham, H. The forward speed diffraction problem. {\em Journal Of Ship Research}. \textbf{42}, 99-112 (1998)
\bibitem{kirby2003aliasing}Kirby, R. \& Karniadakis, G. De-aliasing on non-uniform grids: algorithms and applications. {\em Journal Of Computational Physics}. \textbf{191}, 249-264 (2003)
\bibitem{king1988seakeeping}King, B., Beck, R. \& Magee, A. Seakeeping calculations with forward speed using time domain analysis. (Proc. 17th Symp. on Naval Hydrodynamics,1988)
\bibitem{lee2006wamit}Lee, C. \& Newman, J. Wamit user manual. {\em WAMIT, Inc}. (2006)
\bibitem{lee1995heave}Lee, J. On the heave radiation of a rectangular structure. {\em Ocean Engineering}. \textbf{22}, 19-34 (1995), https://www.sciencedirect.com/science/article/pii/0029801893E0009H
\bibitem{larsen1983open}Larsen, J. \& Dancy, H. Open boundaries in short wave simulations — A new approach. {\em Coastal Engineering}. \textbf{7}, 285-297 (1983), https://www.sciencedirect.com/science/article/pii/0378383983900224
\bibitem{li2021spectral}Li, Z., Bouscasse, B., Ducrozet, G., Gentaz, L., Le Touzé, D. \& Ferrant, P. Spectral Wave Explicit Navier-Stokes Equations for wave-structure interactions using two-phase Computational Fluid Dynamics solvers. {\em Ocean Engineering}. \textbf{221} pp. 108513 (2021), https://www.sciencedirect.com/science/article/pii/S0029801820314207
\bibitem{laskowski2019modelling}Laskowski, W., Bingham, H. \& Engsig-Karup, A. Modelling of wave-structure interaction for cylindrical structures using a spectral element multigrid method. {\em 34<sup>th</sup> International Workshop On Water Waves And Floating Bodies}. (2019)
\bibitem{ma2001finite}Ma, Q., Wu, G. \& Eatock Taylor, R. Finite element simulations of fully non-linear interaction between vertical cylinders and steep waves. Part 2: numerical results and validation. {\em International Journal For Numerical Methods In Fluids}. \textbf{36}, 287-308 (2001), https://onlinelibrary.wiley.com/doi/abs/10.1002/fld.133
\bibitem{monteserin2018nonlinear}Monteserin, C., Engsig-Karup, A. \& Eskilsson, C. Nonlinear Wave-Body Interaction Using a Mixed-Eulerian-Lagrangian Spectral Element Model.  (2018,6), https://doi.org/10.1115/OMAE2018-77692, V009T13A030
\bibitem{mortensen2021simulation}Mortensen, L., Laskowski, W., Engsig-Karup, A., Eskilsson, C. \& Monteserin, C. Simulation of Nonlinear Waves Interacting with a Heaving Body using a p-Multigrid Spectral Element Method.  (2021,6), ISOPE-I-21-3137
\bibitem{patera1984spectral}Patera, A. A spectral element method for fluid dynamics: Laminar flow in a channel expansion. {\em Journal Of Computational Physics}. \textbf{54}, 468-488 (1984), https://www.sciencedirect.com/science/article/pii/0021999184901281
\bibitem{persson2004simple}Persson, P. \& Strang, G. A simple mesh generator in MATLAB. {\em Siam Review - SIAM REV}. \textbf{46} (2004,6)
\bibitem{porter2008solution}Porter, R. The solution to water wave scattering and radiation problems involving semi-immersed circular cylinders.  (2008)
\bibitem{ransley2019blind}Ransley, E., Yan, S., Brown, S., Mai, T., Graham, D., Ma, Q., Musiedlak, P., Engsig-Karup, A., Eskilsson, C., Li, Q., Wang, J., Xie, Z., Venkatachalam, S., Stoesser, T., Zhuang, Y., Li, Q., Wan, D., Chen, G., Chen, H., Qian, L., Ma, Z., Mingham, C., Causon, D., Gatin, I., Jasak, H., Vukcevic, V., Downie, S., Higuera, P., Buldakov, E., Stagonas, D., Chen, Q., Zang, J. \& Greaves, D. A Blind Comparative Study of Focused Wave Interactions with a Fixed FPSO-like Structure (CCP-WSI Blind Test Series 1). {\em International Journal Of Offshore And Polar Engineering}. \textbf{29}, 113-127 (2019,6), https://doi.org/10.17736/ijope.2019.jc748
\bibitem{read2012overset}Read, R. \& Bingham, H. An Overset Grid Approach to Linear Wave-Structure Interaction. (31st International Conference on Offshore Mechanics,2012,7), https://doi.org/10.1115/OMAE2012-83568
\bibitem{read2012solving}Read, R. \& Bingham, H. Solving the linear radiation problem using a volume method on an overset grid. {\em 27<sup>th</sup> International Workshop On Water Waves And Floating Bodies}. (2012)
\bibitem{read2011linear}Read, R. \& Bingham, H. Linear wave-structure interaction using overset grids. {\em 26<sup>th</sup> International Workshop On Water Waves And Floating Bodies}. (2011)
\bibitem{roache2002code}Roache, P. The Method of Manufactured Solutions for Code Verification. {\em Computer Simulation Validation: Fundamental Concepts, Methodological Frameworks, And Philosophical Perspectives}. pp. 295-318 (2019), https://doi.org/10.1007/978-3-319-70766-2%5C_12
\bibitem{robertson1999free}Robertson, I. \& Sherwin, S. Free-Surface Flow Simulation Using hp/Spectral Elements. {\em Journal Of Computational Physics}. \textbf{155}, 26-53 (1999), https://www.sciencedirect.com/science/article/pii/S0021999199963283
\bibitem{taylor1996analysis}Taylor, R. Analysis of Non-Linear Wave-Body Interactions Using Finite Elements. {\em Waves And Nonlinear Processes In Hydrodynamics}. pp. 51-62 (1996), https://doi.org/10.1007/978-94-009-0253-4%5C_4
\bibitem{ursell1949heaving}Ursell, F. On the heaving motion of a circular cylinder on the surface of a fluid. {\em The Quarterly Journal Of Mechanics And Applied Mathematics}. \textbf{2}, 218-231 (1949,1), https://doi.org/10.1093/qjmam/2.2.218
\bibitem{visbech2022efficient}Visbech, J., Engsig-Karup, A. \& Bingham, H. Efficient computation of the linear radiation problem using a spectral element method discretisation. {\em 37<sup>th</sup> International Workshop On Water Waves And Floating Bodies}. (2022)
\bibitem{xu2018spectral}Xu, H., Cantwell, C., Monteserin, C., Eskilsson, C., Engsig-Karup, A. \& Sherwin, S. Spectral/hp element methods: Recent developments, applications, and perspectives. {\em Journal Of Hydrodynamics}. \textbf{30} (2018,2)
\bibitem{zhang2009non}Zhang, W. Non-reflecting simulation for fullynonlinear irregular wave radiation. {\em 24<sup>th</sup> International Workshop On Water Waves And Floating Bodies}. (2009)
\bibitem{zakharov1968stability}Zakharov, V. Stability of periodic waves of finite amplitude on the surface of a deep fluid. {\em Journal Of Applied Mechanics And Technical Physics}. \textbf{9}, 190-194 (1968)
\bibitem{zheng2004radiation}Zheng, Y., You, Y. \& Shen, Y. On the radiation and diffraction of water waves by a rectangular buoy. {\em Ocean Engineering}. \textbf{31}, 1063-1082 (2004), https://www.sciencedirect.com/science/article/pii/S0029801804000095
\bibitem{wu1994finite}Wu, G. \& Eatock Taylor, R. Finite element analysis of two-dimensional non-linear transient water waves. {\em Applied Ocean Research}. \textbf{16}, 363-372 (1994), https://www.sciencedirect.com/science/article/pii/0141118794000298
\bibitem{wu2003coupled}Wu, G. \& Taylor, R. The coupled finite element and boundary element analysis of nonlinear interactions between waves and bodies. {\em Ocean Engineering}. \textbf{30}, 387-400 (2003), https://www.sciencedirect.com/science/article/pii/S0029801802000379
\bibitem{white1994comparing}White, J., Phillips, J. \& Korsmeyer, T. Comparing precorrected-fft and fast multipole algorithms for solving three-dimensional potential integral equations. (Proceedings of the Colorado Conference on Iterative Methods,1994)
\bibitem{AndersThesis}Strom, E. \& Melander, A. Massively Parallel Nodal Discontinous Galerkin Finite Element Method Simulator for 3D Room Acoustics (MSc Thesis). (Technical University of Denmark,2020)
\bibitem{andersen2016floating}Andersen, M. Floating foundations for offshore wind turbines. (Aalborg Universitetsforlag,2016)
\bibitem{bingham1994simulating}Bingham, H. Simulating ship motions in the time domain. (Massachusetts Institute of Technology,1994)
\bibitem{engsig2007unstructured}Engsig-Karup, A. Unstructured nodal DG-FEM solution of high-order Boussinesq-type equations. (Technical University of Denmark, Section of Coastal, Structural,2007)
\bibitem{king1987time}King, B. Time-domain analysis of wave exciting forces on ships and bodies. (University of Michigan,1987)
\bibitem{korsmeyer1988first}Korsmeyer, F. The first-and second-order transient free-surface wave radiation problems. (Massachusetts Institute of Technology,1988)
\bibitem{liapis1986time}Liapis, S. Time-domain analysis of ship motions. (University of Michigan,1986)
\bibitem{Gmsh}Geuzaine, C. \& Remacle, J. A three-dimensional finite element mesh generator with built-in pre- and post-processing facilities. , https://gmsh.info/
\bibitem{DistMesh}Persson, P. \& Strang, G. DistMesh - A Simple Mesh Generator in MATLAB. , http://persson.berkeley.edu/distmesh/
\bibitem{DelaunayTriangulation}Mathworks Delaunay Triangulation. , https://se.mathworks.com/help/matlab/ref/delaunaytriangulation.html
\bibitem{Stiesdal}Stiesdal The TetraSpar full-scale demonstration project. , https://www.stiesdal.com/offshore-technologies/the-tetraspar-full-scale-demonstration-project/
